Active Distribution Grids Providing Voltage Support: The Swiss Case

The increasing installation of controllable Distributed Energy Resources (DERs) in Distribution Networks (DNs) opens up new opportunities for the provision of ancillary services to the Transmission Network (TN) level. As the penetration of smart meter devices and communication infrastructure in DNs increases, they become more observable and controllable with centralized optimization-based control schemes becoming efficient and practical. In this paper, we propose a centralized tractable Optimal Power Flow (OPF)-based control scheme that optimizes the real-time operation of active DNs, while also considering the provision of voltage support as an ancillary service to the TN. We embed in the form of various constraints the current voltage support requirements of Switzerland and investigate the potential benefit of ancillary services provision assuming different operational modes of the DER inverters. We demonstrate the performance of the proposed scheme using a combined HV-MV-LV test system.

==> passive.tex <==
% \documentclass[tightpage,usenames,dvipsnames]{standalone}
% %[]{beamer}
% \usepackage{tikz,pgfplots}
% \usepgfplotslibrary{patchplots}
% \usepackage{myStyleIEEE}
% \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=5cm, minimum height=1cm,text centered, draw=black, fill=red!30]
% \tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=5cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
% \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, text width=3.5cm, draw=black, fill=Gray!30]
% \tikzstyle{decision} = [diamond, aspect=2 ,minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]

% \usetikzlibrary{arrows,positioning}
% \tikzset{
%   mylabel/.style = {font=\footnotesize, midway, fill=white, anchor=center}
% }
% \begin{document}

% \begin{varwidth}{\linewidth}

\centering
\begin{tikzpicture}[node distance=2cm, align=center, scale=1, every node/.style={transform shape}]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% % Draw axes
\draw[<->,thick] (-3,0)--(3,0) node[right,rotate=90] {}; %Xaxis
\draw[<->,thick] (0,-4.5)--(0,4.5) node[right,rotate=90] {}; %Xaxis
\begin{scope}[on background layer]
\fill[blue!20]   (-0.484*4,4)  -- (0.484*4,4) -- (0.484*1,1) -- (0.484*1,-1)-- (0.484*4,-4) -- (-0.484*4,-4) -- (-0.484*1,-1) -- (-0.484*1,1)-- cycle;
\end{scope}
\node (AS) [black, rectangle,inner sep=2pt, align=center, line width=0.2mm] at (0.5,4.5) {$E_{\textrm{P}}$};
\node (AS) [black, rectangle,inner sep=2pt, align=center, line width=0.2mm] at (3,-0.5) {$E_{\textrm{Q}}$};
\node (AS) [black, rectangle,inner sep=2pt, align=center, line width=0.2mm] at (-0.2,-0.2) {$0$};
\node (AS) [black, rectangle,inner sep=2pt, align=center, line width=0.2mm] at (-0.8,3) {Cost-free\\region};
\draw [arrow, dashed][-] (-0.484*4,4) -- (-0.484*1,1) -- (-0.484*1,-1) -- (-0.484*4,-4);
\draw [arrow, dashed][-] (0.484*4,4) -- (0.484*1,1) -- (0.484*1,-1) -- (0.484*4,-4);

\draw [arrow][<->] (0,0.2) -- (0.5,0.2); \node at (1,0.2) {$E_{\textrm{Qlim}}^{\textrm{tr}}$};
\draw [arrow][<->] (0,2) -- (0.484*2,2); \node at (1.7,2) {$E_{\textrm{Qlim}}^{\textrm{pf}}$};

\node [blue] at (-2.5,1.5) {\textbullet};\node [blue] at (-2.5,1.2) {A};
\draw [arrow, blue][<->] (-2.5,1.5) -- (-0.484*1.5,1.5) node[mylabel, pos=0.5] {billed};


\end{tikzpicture}
    
% \end{varwidth}
% \end{document}

